Classifying Copy Number Variations Using State Space Modeling of Targeted Sequencing Data: A Case Study in Thalassemia

Thalassemia, a blood disorder and one of the most prevalent hereditary genetic disorders worldwide, is often caused by copy number variations (CNVs) in the hemoglobin genes. This disorder has incredible diversity, with a large number of distinct profiles corresponding to alterations of different regions in the genes. Correctly classifying an individual's profile is critical as it impacts treatment, prognosis, and genetic counseling. However, genetic classification is challenging due to the large number of profiles worldwide, and often requires a large number of sequential tests. Targeted next generation sequencing (NGS), which characterizes segments of an individual's genome, has the potential to dramatically reduce the cost of testing and increase accuracy. In this work, we introduce a probabilistic state space model for profiling thalassemia from targeted NGS data, which naturally characterize the spatial ordering of the genes along the chromosome. We then use decision theory to choose the best profile among the different options. Due to our use of Bayesian methodology, we are also able to detect low-quality samples to be excluded from consideration, an important component of clinical screening. We evaluate our model on a dataset of 57 individuals, including both controls and cases with a variety of thalassemia profiles. Our model has a sensitivity of 0.99 and specificity of 0.93 for thalassemia detection, and accuracy of 91.5\% for characterizing subtypes. Furthermore, the specificity and accuracy rise to $0.96$ and 93.9\% when low-quality samples are excluded using our automated quality control method. This approach outperforms alternative methods, particularly in specificity, and is broadly applicable to other disorders.

==> texfiles/old_introduction.tex <==
Thalassemia is a hereditary blood disorder that disrupts the body's ability to produce adequate hemoglobin, leading to chronic anemia and severe health complications. As one of the most prevalent genetic disorders worldwide, it poses a significant public health challenge, particularly in regions such as the Mediterranean, Southeast Asia, and sub-Saharan Africa \cite{weatherall2008thalassaemia,modell2008global}. The disease results from copy number variations (CNVs) in the \textit{HBA} (alpha-globin) and \textit{HBB} (beta-globin) genes, where affected individuals have deletions of one or more gene copies. The severity of anemia depends on the number of missing copies, ranging from mild symptoms to life-threatening conditions \cite{galanello2011alpha,cao2010beta,rund2005beta}. Due to the complexity of genetic inheritance, individuals can carry a wide range of thalassemia ``profiles,'' making accurate diagnosis essential for treatment and genetic counseling.

Next generation sequencing (NGS) has revolutionized the diagnosis of such diseases. As a rough description, NGS fragments the individual's DNA into small pieces and then repeatedly duplicates the fragments, amplifying the signal. Finally it sequences all the fragments and reconstructs the sequence of the original material. From a clinical perpective. While whole genome sequencing (WGS) has received the most attention, targeted sequencing that amplifies specific regions provides a cost-effective means of identifying genetic variants associated with diseases \cite{rehm2013disease,ku2013next}. Each target (amplicon) focuses on a specific region of interest, minimizing unnecessary data collection \cite{mamanova2010target}. This method is particularly advantageous in clinical settings where the cost of genetic testing needs to be balanced against the need for accurate and rapid diagnosis \cite{rabbani2012next}. By aggregating the information from each amplicon, we can obtain a full picture of the genomic architecture of the relevant gene.

Unfortunately, CNVs are the most difficult mutation to diagnose via NGS \cite{}. Unlike more well known mutations like single nucleotide polymorphisms, CNVs require evaluating the quantity of reads amplified, as opposed to simply detecting an altered sequence in a significant portion of the reads. Most methods, including ours, function by comparing the amplification observed in the sample to amplification observed in a copy neutral control sample. Due to the difficulty with CNV diagnosis, most methods require either large numbers of samples to be simultaneously analyzed \cite{,,} or that the CNVs extend over large regions of the genome \cite{,,}, both of which are clinically unsuitable requirements. Furthermore, none of these methods profile the type of thalassemia is exhibited by the patient.

In this paper, we introduce a novel approach to estimating the copy ratios of an individual along with profiling the type thalassemia using targeted amplicon sequencing data. This method is based on state space modeling \cite{chopin2020introduction}, which are natural candidates for sequential data (as these amplicons have a spatial ordering along the gene). This allows for the copy number to be estimated at each amplicon, sharing information between adjacent amplicons to reduce variability. Based on these estimates, we use statistical decision theory to profile the associated thalassemia type from a variety of predefined candidates.  Our method provides a comprehensive analysis of the genetic variations associated with thalassemia, offering a detailed estimation of the copy number at each exon.  Furthermore, our method operates within a Bayesian framework, allowing for the incorporation of prior knowledge and the estimation of uncertainty in all predicted quantities. This probabilistic approach not only provides robust and interpretable results but also offers clinicians insights into the confidence level of each prediction, which is essential for informed decision-making in a clinical setting.


\subsection*{Generalizable Insights about Machine Learning in the Context of Healthcare}

\begin{itemize}
    \item Bayesian evidence significantly enhances diagnostic accuracy by identifying low-quality samples that require manual review or rerunning.
    \item Guided particle filtering improves performance in state space models, particularly in scenarios where abrupt changes are expected.
\end{itemize}


==> texfiles/old_methods.tex <==
\subsection {Notation and Data}

We analyze read counts from $J$ amplicons in a sample, denoted as ${s_j}{j=1:J}$, and corresponding normal control counts, ${n_j}{j=1:J}$. To assess copy number variations (CNVs), we compute the log copy ratio for each amplicon $y_j=\log(s_j)-\log(n_j)$ (the read depth is roughly 500 making $\log(0)$ not observed in practice). A subset of these amplicons, located on different chromosomes, serves as controls to correct for systematic biases. To ensure consistency across samples, we normalize the observed values by subtracting the median log ratio across all user-defined control amplicons, which are assumed to be CNV-neutral. In this normalized scale, $y_j = 0$ indicates a copy-neutral amplicon, while negative values suggest deletions and positive values indicate amplifications. Since amplicons are sequentially ordered, we expect adjacent amplicons targeting the alpha or beta genes to exhibit similar copy number ratios.

Thalassemia diagnosis relies on predefined "profiles" that represent expected log ratios for each amplicon. We denote the expected log ratio for the $i$-th profile as $d_i = {d_{ij}}_{j=1:J}$. These profiles vary significantly, often corresponding to specific ancestries such as Southeast Asian or Turkish, and may represent heterozygous or homozygous mutations. Given that each chromosome contains two copies of a gene, possible copy ratios for a loss at any amplicon within an individual are 0, $\frac{1}{4}$, $\frac{1}{2}$, and $\frac{3}{4}$, with similar values for gains. For a given sample, our analysis involves two key tasks:
\begin{enumerate}
    \item Estimating the copy number ratio at each exon
    \item Identifying the most likely thalassemia profile for both the alpha and beta genes.
\end{enumerate}


%We observe read counts from $J$ amplicons in a sample, denoted by $\{s_j\}_{j=1:J}$, and corresponding counts from a normal control, denoted by $\{n_j\}_{j=1:J}$. To assess copy number variations, we compute the log copy ratio for each amplicon as $y_j = \log\left(\frac{s_j + 1}{n_j + 1}\right)$, where the addition of $1$ to both $s_j$ and $n_j$ prevents undefined logarithmic operations. Among these $J$ amplicons, a small subset comprise control amplicons located on different chromosomes, serving to correct for systematic biases between samples. The observed values we analyze are "normalized" by subtracting the median of the log ratios across all user-defined control amplicons, amplicons guaranteed to be CNV-neutral, ensuring consistency across samples. In this normalized scale, $y_j = 0$ indicates a copy-neutral amplicon, with negative values reflecting deletions and positive values indicating amplifications. The amplicons are ordered sequentially, by extension we expect copy number ratios to be similar for adjacent amplicons in the alpha gene and similarly for amplicons  targeting the beta gene.

%We are provided with a set of potential ``profiles'' for thalassemia, representing the expected log ratios for each amplicon. We denote the expected log ratio for the $i$-th profile as $d_i = \{d_{ij}\}_{j=1:J}$. These profiles can vary significantly and are often associated with specific ancestries, such as Southeast Asian, Turkish, or more general categories like an alpha 3.7 loss/gain. These variations can manifest as either heterozygous or homozygous mutations. Considering that each chromosome contains two copies of a gene, the possible copy ratios for a loss in any amplicon within a specific individual are 0, $\frac{1}{4}$, $\frac{1}{2}$, and $\frac{3}{4}$, with similar ratios applicable for gains. For a given sample we then have two tasks, (i) estimate the copy ratio at each of the exons and (ii) provide a profile for both the alpha and beta genes.


\subsubsection{A State Space Model of the Log Copy Ratios}

Given the strong spatial correlations expected in this context, we anticipate that the true copy number ratio, denoted as $x_j$, will be highly correlated between adjacent amplicons. A natural way to model this relationship is through a state-space framework \cite{chopin2020introduction}, where the empirical log copy ratios are treated as noisy observations of the underlying true log copy ratios. Correlations in the unobserved space are induced by modeling the true copy ratios as a Markov chain. Estimating these copy ratios is then achieved by computing the posterior distribution $p(x \mid y)$, where $y$ represents the observed log copy ratios.

In most genomic regions, we expect the log copy ratio to remain constant, with occasional large shifts due to CNVs. To capture this behavior, we define a transition kernel as a Gaussian mixture model:

\begin{equation}\label{eq:transition_kernel} p(x_{j+1} \mid x_j) = (1-p) \mathcal{N}(x_j, \epsilon) + p \mathcal{N}(x_j, \sigma^2), \end{equation}

where $\sigma^2 \gg \epsilon$ and $p \approx 0.01$. This formulation reflects the expectation of rare but significant jumps in copy number. Although setting $\epsilon=0$ would be more biologically justifiable—implying that true CNVs only change in discrete steps—doing so significantly degrades inference quality, as discussed later.

To enhance robustness against outliers, we use a Laplace observational likelihood. Additionally, we impose a weak prior on the first amplicon, assuming it to be copy-neutral. The complete probabilistic model is defined as:
\begin{equation}\label{eq:state_space_model} 
\begin{split} 
p(x_0) &= \mathcal{N}(0, \tau), \\ 
p(x_{j+1} \mid x_j) &= (1-p) \mathcal{N}(x_j, \epsilon) + p \mathcal{N}(x_j, \sigma^2), \\ 
p(y_j \mid x_j) &= \text{Laplace}(x_j, b). 
\end{split} 
\end{equation}

Here, $p$, $\epsilon$, $\sigma^2$, and $b$ are tunable parameters chosen by the user with natural inrepretations. 
\begin{itemize}
\item $p$ controls the probability of a jump in copy number; larger values allow for more frequent changes.
\item $\sigma^2$ determines the magnitude of copy number changes.
\item $b$ governs the noise level in the observed copy number ratios, with larger values indicating lower confidence in any specific estimate.
\item $\epsilon$ is a small stabilizing term that prevents inference issues, ensuring smooth transitions between jumps rather than enforcing strict constancy.
\end{itemize}

%Given the strong spatial correlations expected in this context, we anticipate that the true copy number ratio, denoted as $x_j$, will be highly correlated between adjacent amplicons. A natural approach to capture this correlation is through a state space model \cite{chopin2020introduction}. In this framework, we model the empirical log copy ratios as noisy observations of the unobserved true log copy ratios. We induce correlations in the unobserved space by modeling the true copy ratios as a Markov chain. Estimating the copy ratios for the amplicons is then achieved by computing the posterior distribution $p(x \mid y)$, where $y$ represents the observed log copy ratios.

%Based on the application, we expect that the log copy ratio remains constant in most regions, with occasional large jumps due to CNVs. To model this, we use a transition kernel defined as a Gaussian mixture model, 
%\begin{equation}\label{eq:transition_kernel}
%p(x_{j+1} \mid x_j) = (1-p) \mathcal{N}(x_j, \epsilon) + p \mathcal{N}(x_j, \sigma^2),
%\end{equation}
%where $\sigma^2 \gg \epsilon$ and $p \approx 0.01$. This setup captures the expectation of rare but significant changes in copy number. While $\epsilon=0$ is more biologiacally justifiable (no variation in true CNV asides from discrete jumps), such an approach dramatically degrades inference as discussed later. Additionally, we employ a Laplace observational likelihood to ensure robustness against outliers. Finally, we place a weak prior on the first amplicon, assuming it to be copy-neutral. The resulting probabilistic model is expressed as:
%\begin{equation}\label{eq:state_space_model}
%\begin{split}
%p(x_0) &\sim \mathcal{N}(0, \tau), \\
%p(x_{j+1} \mid x_j) &\sim (1-p) \mathcal{N}(x_j, \epsilon) + p \mathcal{N}(x_j, \sigma^2), \\
%p(y_j \mid x_j) &\sim \text{Laplace}(x_j, b).
%\end{split}
%\end{equation}
%In this formulation $p$, $\epsilon$, $\sigma^2$ and $b$ are tuning parameters that can be chosen by the user. The interpretations are as follows: $p$ represents the probability of a jump occurring, larger values allow for a greater number of changes in copy number estimates. Larger values for $\sigma^2$ allow for greater changes in copy number, while the value of $b$ corresponds to how ``noisy'' the empirical copy number ratios are. Larger values indicate lower confidence in any particular copy ratio. Finally, $\epsilon$ is a small number meant to improve algorithmic stability as opposed to $0$ indicating a constant copy number ratio between jumps.

\subsubsection{Inference Via Sequential Monte Carlo}
\label{ssec:sequential_mcmc}

In this subsection, we provide the basics of sequential Monte Carlo, also known as particle filtering, required to fully describe our inference algorithm for \eqref{eq:state_space_model}. The breadth and complexity of this field makes any such undertaking inherently insufficient. We strongly encourage reading Chapters 5, 8, 10, and 11 of \citet{chopin2020introduction} whose notation we match in this section.


The state space model defined in \eqref{eq:state_space_model} does not provide a simple formula for the distribution of the copy ratios given the empirical copy ratios, that is $p(x\mid y)$. A common approach in Bayesian inference is to use Monte Carlo methods \cite{robert2004monte}, which draw samples from the posterior distribution and use these samples to approximate the quantities of interest (i.e. means, medians, quantiles). Often, drawing samples from these distributions is intractable as well. In such circumstances, we can construct a Markov chain that converges to the posterior distribution \cite{}. We use samples from this chain as approximate samples from our posterior.

Unfortunately, traditional methods \cite{betancourt2017conceptual} are poorly suited to state space models due to the intense correlations introduced by the unobserved latent space. Functionally the space is high dimensional making the variance in MCMC estimates unacceptable in all but the shortest of sequences \cite{chopin2020introduction}. Sequential Monte Carlo exploits the Markov aspect of the state space models ($x_{j+1}$ depends solely on $x_j$), to dramatically improve the quality of estimates.

The basic algorithm works as follows. First, $N$ samples or ``particles'' are generated from the prior distribution $X_0^N\sim p(x_0)$. We then weight these particles based on how well these data align with the observed ratio $w_0^N=p(y_0|X_0^N)$ and normalize by the total weights $W_0^N=w_0^N/\sum_{i=1}^N w_0^i$. In other contexts, this is known as importance sampling \cite{robert2004monte} with auto-normalization. We then ``resample'' these particles according to their weights $A_0^{1:N}=\text{resample}(W_0^{1:N})$, particles with large weights are more likely to be kept than particles with low weights as these particles are more likely based on the data. Finally, samples at the next step are generated according to the transition kernel $X_1^N\sim p(x_1\mid X_0^{A_0^N})$. This process repeats for the entire sequence $J$ times. Each iteration generates a set of samples $X_j^N$ and weights $W_j^N$ that will be used to approximate the relevant quantities (such as the posterior median of the copy number ratio). The algoithm is provided in Algorithm \ref{alg:pf}.

\begin{algorithm2e}[h]
\caption{Standard Particle Filter}
\KwData{Observations $y_0, \dots, y_J$}
\KwResult{Particles $X_j^n$ and weights $W_j^n$}
\For{$n \leftarrow 1$ \KwTo $N$}{
    Sample $X_1^n \sim p_0(x_0)$\;
    $w_1^n \gets p(y_0 \mid X_0^n)$\;
}
Normalize $W_1^n = w_1^n / \sum_m w_1^m$\;

\For{$j \leftarrow 2$ \KwTo $J$}{
    $A_j^{1:N} \gets \text{resample}(W_{j-1}^{1:N})$\;
    \For{$n \leftarrow 1$ \KwTo $N$}{
        $\hat{w}_{j-1}^n \gets 1$\;
        Sample $X_j^n \sim p(x_j \mid X_{j-1}^{A_j^n})$\;
        $w_j^n \gets \hat{w}_{j-1}^n p(y_j \mid X_j^n)$\;
    }
    Normalize $W_j^n = w_j^n / \sum_m w_j^m$\;
}
\end{algorithm2e}


The samples from \ref{alg:pf} are sufficient to estimate the copy number ratio at amplicon $j$ given the preceding copy number ratios, that is $p(x_j\mid y_{0:j})$, however, this is not the distribution of interest. Rather, we wish to characterize the distribution on the copy number ratio given observed copy ratios, $p(x_j\mid y_{0:J})$. In spite of their superficial similarity, the latter task is substantially more difficult and requires an additional step known as ``backward smoothing''.  There are multiple algorithms for approximating this distribution, in this work we use a  method known as the two-filter method described in Chapter 12 of \cite{chopin2020introduction}. 

We know that the distribution of $p(x_T\mid y_{0:T})$ can be computed directly from the weights obtained by the forward filter, $W_T^N$. We can obtain the marginal distribution of the discrete particles for $(X_{T-1},X_T)$ using the backward transition density. We can integrate out the particles $X_T$ to obtain backward weights $W_{t\mid T}^N$ used for importance sampling estimates of statistics of $p(x_t\mid y_{0:T})$. The algorithm is provided in  \eqref{alg:backward_smoothing}



Finally, one issue with the standard (or ``bootstrap'') filter described above is that many of the samples from the transition kernel will be close to the current value, that is $X_{j+1}^n\approx X_j^n$. This is due to how the model was designed the transition kernel \eqref{eq:transition_kernel}; we expect that an abrupt change in copy ratio should be infrequent. However, this means that when the true ratio does change, very few particles will be generated near the new value, resulting in poor uncertainty quantification, or in extreme cases failure to detect the shift in copy ratio entirely. We can solve this issue by introducing a ``guide'' to encourage samples to be drawn over a greater rangel That is, rather than generating samples from $p(x_j\mid x_{j-1})$ we generate samples from the guide $q(x_j\mid x_{j-1})$ to artificially increase the probability of samples away from the current value. As long as the distribution for computing the weights ``inverts'' the change introduced by sampling from a different transition distribution, as described in Chapter 12 of \citet{chopin2020introduction}, the samples will still approximate the posterior (but with superior properties). In our work we use a Gaussian mixture model as a guide
\begin{equation}\label{eq:guide}
 q(x_j\mid x_{j-1})=\sum_{i=1}^5 0.2 \mathcal{N}(c_i+x_{j-1},3\sigma^2),
\end{equation}
where $c_i=\{-1,-0.5,0,0.5,1.0\}$. As we demonstrate in section \ref{ssec:guide}, this guide is critical in proper evaluation of sample quality and improves CNV estimation.

\subsubsection{Profiling via Bayesian Decision Theory}

To this point, our focus has been on estimating the copy number at each amplicon. This is an important intermediate step, but not our final goal of profiling the thalassemia type. We now develop our method for assigning a specific predefined profile to a sample, denoting the disease status as $D$. The diagnoses $d_i$ mentioned in the introduction represent the expected log ratio of any individual that matches the profile, that is $d_{ij}=E[x_i\mid D=i]$. We can convert this into a probabilistic model by placing a distribution of the true copy number $x_j$ conditioned on the expected value of the disease, $d_{ij}$. In this work, we will use a normal disturibution, $p(x_j|D=i)= N(d_{ij},\phi^2)$. If we had access to the true copy number, we could provide an optimal \cite{} prediction of profile as 
\begin{equation}\label{eq:optimal}
\hat{D}=\arg\max_{i} \prod_{j=1}^J p(x_j|D=i)p(D=i)
\end{equation}
Unfortunately, we do not have access to the true copy ratios, only the empirical copy ratios, making \eqref{eq:optimal} not directly usable. However, we can obtain the distribution of the diagnoiss conditional on these empirical ratios by integrating out the estimates of the true copy ratio as 
\begin{equation}
    p(D=i\mid y_{1:J})=\int p(D=i\mid x_{1:J})p(x_{1:J}\mid y_{1:J})dx_{1:J}.
\end{equation}
The first distribution is known by definition and approximating the latter distribution was the focus of Section 
In practice, given samples from our backward smoothing algorithm, approximating this distribution is straightfoward. For each trajectory, simply evaluate  $p(D=i\mid x_{1:J})$ and take the average. From this point, choosing a profile is straightforward deciding which profile has the highest probability.


There is one fudge factor required for this to work in practice. When an individual possesses a homozygous deletion they will have zero, or a very tiny number of counts in the specific amplicon. This violates an assumption made implicitly in using the log copy ratios; that the read depths are large enough to be considered approximately continuous.  
  



\subsubsection{Sample Quality Evaluation via Model Evidence}
\label{ssec:quality_score}

Finally, a key concern in many clinical applications is determining whether a sample meets the quality standards necessary for making a reliable diagnosis. It is important to note that this is distinct from having an ``uncertain'' high-variance posterior. Intuitively, an ambiguous opinion after observing high-quality data is very different from uncertainty from low quality data. Any probabilistic model, such as ours defined in \eqref{eq:state_space_model}, provides a natural way to assess the latter, as how "realistic" the observed data are according to the model. This is done using the model likelihood (or normalization constant) as a measure of fit. However, computing this normalization constant is generally non-trivial, as most inference methods—such as MCMC—are designed to bypass its direct computation. Fortunately, the particle filter offers a straightforward estimator: the mean of the unnormalized importance weights, given by

\begin{equation} \ell_j = \frac{1}{N}\sum_{i=1}^N w_i. \end{equation}

The total normalization constant for a sample is then computed as the product of these individual normalization constants:

\begin{equation} L=\prod_{j=0}^J \ell_j. \end{equation}

While $L$ provides a measure of model fit, its absolute value is somewhat arbitrary, as it is expressed in "nats" of information. Additionally, simple parameter choices, such as $b$ or $\sigma^2$, can significantly influence these values. However, $L$ is useful for comparing samples: a low value relative to other samples suggests that the state-space model is a poor fit for that particular sample. This provides a natural quality control mechanism—samples with low likelihood scores should be flagged and returned to the clinician for manual review.

As previously noted, high-quality samples containing homozygous deletions can violate model assumptions, leading to artificially low values of $L$. To mitigate this issue, we use a more robust metric: the median of the individual likelihood values

\begin{equation} QC = \text{Median}({\ell_j}_{j=0:J}). \end{equation}

The median is resistant to outliers \cite{ronchetti2009robust}, allowing us to evaluate sample quality based on a typical amplicon. We set a threshold for rejecting samples: those with a $QC$ score more than three standard deviations below the mean are considered low quality and excluded from further analysis.

%Finally, a major concern in many clinical applications is deciding whether the sample quality is sufficient in order to make a diagnosis. The probabilistic model defined in \eqref{eq:state_space_model} provides a natural means for quantifying how ``realistic'' the data are according to the model in terms of the model likelihood or normalization constant. In general, computing the normalization constant is non-trivial, and most inference methods, such as MCMC,b m are techniques designed to avoid its explicit computation. Fortunately, the particle filter provides a natural estimtor, namely the mean of the unnormalized importance weights
%\begin{equation}
%    \ell_j = \frac{1}{N}\sum_{i=1}^N w_i.
%\end{equation}
%The total normalization constant is simply the product of these normalization constants $L=\prod_{j=0}^J \ell_j$. 

%For each sample $L$ is a somewhat arbitrary number, (its units are ``nats'' of information). Simple decisions on parameters such as $b$ or $\sigma^2$ can dramatically alter these numbers. However, they provide a natural means to \textit{compare} samples; a low value of $L$ compared to other samples is indicative of the state space model being a poor fit for that specific sample. Thus, this provides a natural means to perform quality control in profiling; the diagnoses associated with low likelihoods \textit{should} be ignored and returned to the clinician for manual review. As mentioned previously, high quality samples with homozygous deletions violate model assumptions and will result in low values of $L$. To avoid this, we use as a metric the median of the values
%\begin{equation}
%    QC = \text{Median}(\{\ell_j\}_{j=0:J}).
%\end{equation}
%The median is robust to these outliers \cite{ronchetti2009robust}, allowing us to evaluate the sample quality with respect to an ``average'' amplicon. We choose to reject samples whose $QC$ score is more than three standard deviations below the mean.



==> texfiles/old_results.tex <==


\subsection{Overall Study Objectives} 
There are two overall objectives in this section; first, we wish to evaluate the accuracy of our thalassemia profiling and second, we wish to evaluate the ability of Bayesian evidence to recognize substandard samples. To evaluate the former, we use the dataset described in ???. Unfortunately, as previously mentioned, we have no competitor methods to contrast our performance. For the latter, we use data from a similar panel designed for detecting BRCA mutations. It contained 283 amplicons: 20 control amplicons, 149 targeting specific regions on the BRCA2 gene, and the remainder targeting the BRCA1 gene. Once again, each sample underwent targeted sequencing on Illumina’s MiSeq platform, with an average coverage of approximately 2,600 read pairs per amplicon. The dataset included 77 samples across 5 batches, comprising 40 cell line positives, 27 cell line normals, and 10 Formalin-Fixed, Paraffin-Embedded (FFPE) positives. The FFPE processing causes DNA degradation, leading to erratic empirical copy ratios when an unmatched (non-FFPE) cell line normal is used as a reference for an FFPE sample. Thus, the FFPE samples serve as known "poor-quality" samples, allowing us to evaluate the quality score’s effectiveness in distinguishing between cell line and FFPE samples.

\subsection{Evaluating Profile Accuracy}
\label{ssec:profile_accuracy}

We first evaluate our ability to classify thalassemia profiles. We first evaluate the ability of our algorithm to distinguish cases from controls, without profiling the specific type of genetic mutation. We were able to artificially increase sample size by using 4 different runs with two distinct normal samples to profile thalassemia in the samples. The resulting augmented data included 220 sample/normal pairs.   We found that our algorithm yielded a sensitivity of 98.9\% and a specificity of 65.9\%, as shown on the left of Table \ref{tab:results_thal}. However, we found that many of our false positives were from samples that were considered poor quality based on the generative likelihood. When we filtered out the samples that failed our QC metric introduced in Section \ref{ssec:quality_score}, the sensitivity was unaltered but the specificity rose to 78.1\% due to a reduction of false positives from 15 to 7, as shown on the right.

We then evaluated the predictive ability of our model to profile the specific profile of thalassemia. We considered 28 potential profiles of thalassemia, involving heterozygous and homozygous combinations of different common subtypes observed. Unfortunately, two of the mutations in the dataset, the large HBA duplication and the alpha-4.2 duplication/alpha-3.7 deletion are outside the scope of considered diagnoses and are ommitted from this portion of the analysis. We found that without any form of quality control we obtained an accuracy rate of 86.8\% while with quality control the accuracy rate improved to 91.5\%. A visualization of this process is shown in Figure \ref{fig3} with three representative samples.

\begin{table}[ht]\label{tab:results_thal}
\centering
\begin{tabular}{c|c|c|c|c}

\multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{No QC}} & \multicolumn{2}{c}{\textbf{QC}} \\ %\hline
\textbf{Prediction} & \textbf{Labeled Positive} & \textbf{Labeled Negative} & \textbf{Labeled Positive} & \textbf{Labeled Negative} \\ 
\hline
\textbf{Positive} & 174 & 15 & 167 & 7 \\ \hline
\textbf{Negative} & 2 & 29 & 2 & 25 \\ \hline
\end{tabular}
\caption{Comparison of sensitivity and specificity both with filtering on the quality score (QC) and without such filtering (No QC)}
\end{table}

\begin{figure}[h]
\centering
\includegraphics[width=1.0\textwidth]{figures/ProfileComparisons.pdf}
\caption{The figure presents copy number ratio profiles for three representative sample. On the left, the model correctly predicts a heterozygous alpha-3.7 deletion, with the per amplicon smoothed ratio closely tracking the expected trajectory with a 3.7 deletion shown in black. The model also correctly predicts a homozygous alpha-3.7 deletion in the middle plot, however, the estimated copy ratio has difficulty in estimating a CNR of precisely 0. Finally, tn the third case, the predicted profile (south east Asian) diverges from the true profile, an alpha-3.7 deletion. The predicted profile clearly diverges from the estimated CNV ratio, however, based on the empirical ratios the deletion is wider and more uniform than would be expected due to an alpha-3.7 deletion.}\label{fig3}
\end{figure}

\subsection{Amplicon-Level CNV Estimation}
\label{ssec:amplicon_accuracy}

We now evaluate the the ability of our model to estimate the CNR on an amplicon-by-amplicon basis, as specific amplicons or exons may be of interest in addition to predefined profiles. We can reuse the experimental setup from the previous section, except now we will compare the output of the state space model $p(x|y)$ to the true values defined by the known profiles. We use as our prediction of CNR the exponentiated posterior mean of the log copy ratio and our metric is the root mean squared error of the entire sequence. 

The results are shown in Figure \ref{fig:ampliconaccuracy}. We can see that an an amplicon-by-amplicon basis most of the estimates lie within $0.1$ of the true copy ratio. There are several outliers, but these are filtered by our quality control metric. This also provides an estimate of our limit of detection, we cannot estimate CNR closer than roughly $0.1-0.2$ depending on the level of certainty desired. This is more than sufficient for our purposes, as our samples are almost pure with trisomies and deletions; however, using this model for liquid biopsy where the sample component leads to potential cases where our model would miss a CNV call.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\textwidth]{figures/AmpliconAccuracy_New.pdf}
\caption{The figure on the left plots a histogram of the RMSE of amplicon-level predictions among the thalassemia samples used. The distribution has a large mode between $0.05$ and $0.15$, indicating that most amplicon-level estimates are less than $0.15$ away from the true copy ratio. However, there are several outliers with dramatically elevated deviations from the true copy number ratio. We can see on the plot on the right that these are removed however, by our quality control process.}\label{fig:ampliconaccuracy}
\end{figure}


\subsection{Evaluating the Sample Quality Metric}
\label{ssec:quality}

Finally, we evaluate the ability of our model to detect poor-quality samples for quality control. While we already have evidence for its efficacy due to it dramatically improving specificity in Section \ref{ssec:profile_accuracy}, here we quantify its performance in differentiating between known low-quality samples from higher quality samples.  For this purpose, we use data from a second panel designed to detect SNPs and CNVs in the BRCA1 and BRCA2 genes. This panel was designed to function with two types of samples, liquid biopsy (LBX) and Formalin Fixed and Parrafin Embedded (FFPE) samples. The latter process results in substantial DNA degradation, making the samples viable only for SNP detection. We will fit our model on both types of samples using our model and evaluate the ability to indicate that the FFPE samples are low quality according to the criterion described in Section \ref{ssec:quality_score}.

To evaluate this, we ran our algorithm on 77 samples, 40 were liquid biopsy samples with known mutations (NIST samples), 27 were synthetic normals (TV), and 10 were FFPE samples. We used 3 TVs as normals. The results are shown in Figure \ref{fig:samplequality}. We can see that the empirical copy ratios are far more erratic in the FFPE samples as compared to the clinical samples. This is reflected in the quality scores obtained; the average score for the TV samples and clinical samples  are $0.13\pm 0.01$ and $0.10\pm0.01$ respectively while the scores for the FFPE samples are $-0.76\pm0.02$. From this, we can see a clear separation between the a priori ``low-quality'' samples and the samples that match model assumptions. Based on the quality metric introduced in the methods, all samples from FFPE would have failed quality control and failed to produce a call. By contrast, only a single sample from the cell line positive would have been falsely rejected as being substandard.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\textwidth]{figures/SampleQuality_newGuide.pdf}
\caption{This figure visualizes the sample quality differences detected by our metric. On the left, we show the CNRs of an FFPE sample with a cell-line normal. These ratios fluctuate wildly between $0.5$ and $1.5$, with a standard deviation of $0.6$. In comparison, one of the cell line positives shown in the middle plot has substantially reduced noise in the CNRs, with a standard deviation of $0.16$. Finally, on the right we visualize the QC score standardized by batch to remove run-specific variability. We can see that the FFPE positive samples are all below $-0.5$, while both positive and normal cell-line samples were above this threshold.}\label{fig:samplequality}
\end{figure}
